TorchCraft: a Library for Machine Learning Research on Real-Time Strategy Games

We present TorchCraft, a library that enables deep learning research on Real-Time Strategy (RTS) games such as StarCraft: Brood War, by making it easier to control these games from a machine learning framework, here Torch. This white paper argues for using RTS games as a benchmark for AI research, and describes the design and components of TorchCraft.

==> content/usage.tex <==
\section{Usage}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

% basically follow a simple example to connect to
% torchcraft, line by lane

